Towards blockchain-based robonomics: autonomous agents behavior validation

The decentralized trading market approach, where both autonomous agents and people can consume and produce services expanding own opportunities to reach goals, looks very promising as a part of the Fourth Industrial revolution. The key component of the approach is a blockchain platform that allows an interaction between agents via liability smart contracts. Reliability of a service provider is usually determined by a reputation model. However, this solution only warns future customers about an extent of trust to the service provider in case it could not execute any previous liabilities correctly. From the other hand a blockchain consensus protocol can additionally include a validation procedure that detects incorrect liability executions in order to suspend payment transactions to questionable service providers. The paper presents the validation methodology of a liability execution for agent-based service providers in a decentralized trading market, using the Model Checking method based on the mathematical model of finite state automata and Temporal Logic properties of interest. To demonstrate this concept, we implemented the methodology in the Duckietown application, moving an autonomous mobile robot to achieve a mission goal with the following behavior validation at the end of a completed scenario.

==> general_prototype.tex <==
\section{General prototype description}
\label{sec:gen_prototype}
It is required to develop real-life scenario, including some service (e.g. transportation from one point to another), customer, executive and validator. Also, it is preferable to find case with a chain of service providers, that is, for instance human customer orders some service from Robot1, than Robot1 has to order some other service from Robot2 in order to finish serving its client.
\subsection{Taxi service}
Since mobile robots are widely used and can represent real case - transportation, it was decided to consider taxi service prototype. It is possible to sequentially increase complexity of the prototype by adding new components. Each component and case is a subject for further researches and investigations. In this section we consider each of them on basic level to create background for discussion.
\subsubsection{Basic car order}
The simplest case is to provide ability to create car's liability to move to some point. In that case simple application can accept car's Ethereum account address (which should be known by user in advance) and destination point. Than this application creates liability, which is executed by the car. Liability can be marked as done, if car reaches the destination point. \par
This case is very limited and in real life can be considered as follows: user flags a taxi and have to specify only the destination point.
\subsubsection{Car order from point A to point B}
The next case represents typical scenario of taxi usage. User asks taxi service to pick him from the point A and to go to the point B. One of possible solutions is to create two smart contracts - first for moving from current car position to A point, the second for moving from the A point to the B point. It is reasonable to make cost of the first contract equal to penalty charge, if the user rejects further trip. In that case, the second contract should cost the full service price minus cost of the first contract.\par
The second option is to not "hide" costs from the user and calculate both contracts' cost, depending on destination from the taxi current point to A and from A to B. However, it mostly depends on economic model, not the technical implementation.
\subsubsection{Taxi dispatching service}
In previous cases it was assumed, that user knows car's address in advance. However, usually, there is centralized taxi service, which connects clients and taxi cars with each other. It also possible to implement such model in considered prototype. \par
For instance, there could be taxi service, which can have some nice web-portal or mobile application (like current services have) and liabilities with taxi cars. According to this liabilities taxi service is obliged to provide orders for cars. The simplest way to implement this - create new liability, when the car is vacant. When the client is found, liability should be considered as executed. Car's liability is created between car and user. However, it is also possible to make liability between the user and the service, than between the service and the car.
\subsubsection{Road dispatching service}
The route planning was not considered in previous cases. It can be assumed, that car makes it itself. However, it is also possible to use some external service, providing routes, taking into accounts current road conditions. Liabilities between cars and service also can be created, for instance, for providing route with some time requirements. Liability can be considered as executed, if provided route satisfied requested requirements.
\subsubsection{External validator}
In basic AIRA concept it is assumed, that the validation is based on a log, which is produced by the promisor itself. It means, that validation protects from fault, not from cheating. AIRA relies on reputation system to deal with this problem. However, one of possible improvements can be "hardware validation infrastructure". \par
Road infrastructure can include vehicle-detection devices (for instance, cameras with license plate recognition, or RFID scanner), which can log, that at the specific time the concrete vehicle was located in some location. This information could be published to blockchain and can be used by a liability validator, as additional to the car's log. \par
In that case it makes sense to consider this infrastructure as an agent in economics system, providing validation results not for free. However, in the basic idea it is expected, that liability validators should not spend any funds on validation. In that case it is possible either to reconsider validation mechanism or to engage promisors to pay and get information from road validators. For instance, a car can include price of validator's information in the liability, increasing credibility. During its trip it can detect road validators and pay them for location confirmation.
% * <alexandr.kolotov@gmail.com> 2018-01-29T21:13:55.000Z:
% 
% > However, in the basic idea it is expected, that liability validators should not spend any funds on validation.
% Вот это мне не очень понятно.
% 
% ^.
\subsubsection{Unexpected cases}
Hereinbefore we considered ideal cases, when a passenger goes from point A to point B without accidents and without changing his mind. However, in real life user can ask to change destination point (or even try to leave the car) in the middle of the way. In basic model it means, that initial liability will be marked as unexecuted and car will not receive its payment.\par
To get through this problem it is possible to include in objective's model user's presence sensor. If user unexpectedly leaves the car, it can commit the result and liability will be marked as executed. \par
If user wants to stop the trip or to change it, he can ask the car to do that. The simplest solution is to create new contract - from the stop point to the new destination. Cost of this contract should also include cost of the first part of the route. Only after second contract is created and paid, the first contract can be closed. In that case user should have reserved funds, because he should pay for new contract before he gets funds from the previous one.
\par More complicated and interesting solution is to create new contract and add reference to the old one's log. Model takes into account, that the first contract should be marked as executed, if the second one was confirmed. To overcome the trip price difference problem, the second contract can have price of this difference (even more - negative difference). Validation, based on other contracts and negative cost of liability currently are not considered in AIRA prototype, and, probably should be taken into account.

==> kripke_structure.tex <==
\subsection*{Kripke Structure}
A Kripke structure \cite{KRI63} is usually considered as a convenient way of the software and hardware model representation to further application of the verification procedure by a model checker tool. Thus in order to apply Model Checking for the verification of AS, it is necessary to formally define a Kripke structure from $\mathcal{G} = (\mathcal{A}, \mathcal{V}, \mathcal{V}_{init}, c, \mathcal{OP}, \mathcal{EV})$.

A \textit{Kripke structure} corresponding to an agent-based system $\mathcal{G}$ is a tuple $K_{\mathcal{G}} = (S, S_0, \delta, AP, L)$ where $S$ is a finite set of states; $S = \mathcal{V}$; $S_0$ -  a set of initial states, $S_0 = \mathcal{V}_{init}$; $\delta: S \rightarrow S$ is a transition operator, $\delta = \mathcal{EV}$; $AP$ is a set of propositions; $L: S \rightarrow 2^{AP}$ is a label function that assigns the set of propositions to each state. Label function is defined by representing each proposition as first order predicates over the attributes of $\mathcal{G}$.

The objective of the Model Checking is ensuring that the model represented by the Kripke structure $K_{\mathcal{G}}$ satisfies a property defined in terms of Temporal Logic \cite{CLA86}.
